Self-Stabilizing Balancing Algorithm for Containment-Based Trees

Containment-based trees encompass various handy structures such as B+-trees, R-trees and M-trees. They are widely used to build data indexes, range-queryable overlays, publish/subscribe systems both in centralized and distributed contexts. In addition to their versatility, their balanced shape ensures an overall satisfactory performance. Re- cently, it has been shown that their distributed implementations can be fault-resilient. However, this robustness is achieved at the cost of un-balancing the structure. While the structure remains correct in terms of searchability, its performance can be significantly decreased. In this paper, we propose a distributed self-stabilizing algorithm to balance containment-based trees.

==> edgeswapping.tex <==

\section{Balancing Tree with Edge Swapping}
\label{sec:contribution}


Intuitively a node $n$ is unbalanced if (at least) two of its children have too different heights.
Let $t$ be the ``tall'' one and $s$ the ``small'' one.
Without loss of generality, let's consider that $t$ is the taller children of $n$ and $s$ the smaller.
$n$ would be better balanced if it could find a replacement for $s$; a ``taller'' one.
The point is that height's definition and degree constraint ensures that such node exists in the subtree rooted by $t$.
Without loss of generality, some (at least one) children of $t$ is taller than $s$.
Let one of this node be $u$.
If $n$ swaps/exchanges $s$ and $u$, then it is ``better'' balanced.




==> lowerbound.tex <==


\section{Lower Bound}

\begin{lemma}
 There exists an infinite family of initial configurations for which some execution of the protocol takes at least
$\left\lceil\frac{n}{2}\right\rceil$ rounds, where $n$ is the number of nodes.
\end{lemma}
\begin{proof}
 For odd~$n=2k+1$, let $\calI_n$ be the configuration with~$n$ nodes defined as follows: Nodes $u_1,\dots,u_{k+1}$ form
a directed path with $u_1$ being the root of the tree and, for each~$i$ in the range~$k+2\leq i\leq 2k+1$, node~$u_i$
is a child of node~$u_{i-(k+1)}$. The initial height value of nodes~$u_{k+2},\dots,u_{2k+1}$ is~$0$. For each~$i$ in the
range~$1\leq i\leq k+1$, the initial height value of node~$u_i$ is~$n+2-2i$.
 
 We use a scheduling in which all enabled nodes are activated in each step, therefore each round consists of exactly
one step. It is sufficient to prove that, for each of the first~$k+1$ steps, node~$u_1$ performs a height update. This
follows from the following stronger claim:
%
%\begin{claim*}
\begin{claim}
 For all~$s$, $0\leq s\leq k$, after~$s$ steps, nodes $u_1,\dots,u_{k+1-s}$ form a directed path originating
from~$u_1$, they are all enabled for a height update, and, for each~$i$, $1\leq i\leq k+1-s$, the height of~$u_i$
is~$n+2-2i-s$.
%\end{claim*}
\end{claim}
\begin{proof}[Proof of Claim]
 By induction on~$s$. Note that, in the initial configuration, node~$u_{k+1}$ is a leaf and its height value is~$1$,
therefore it is enabled for height update. Moreover, each node in the path~$u_1\rightsquigarrow u_k$ is enabled for a
height update, since it has a height value that differs by two from the height value of its successor in that path, and
its other child is a leaf with height value~$0$. We conclude that the claim is true for~$s=0$ by construction.

 Assume, now, that the claim is true for all~$s\leq j$, where $0\leq j\leq k-1$. By the inductive hypothesis and the
definition of the scheduler, nodes~$u_1,\dots,u_{k+1-(j+1)}$ perform height updates during the first~$j$ steps,
therefore their children sets are the same as in the initial configuration~$\calI_n$. Moreover, since after~$j$ steps
they are all enabled for height updates, their children set will remain the same after the $(j+1)$-st step. This
implies that after~$j+1$ steps they will still form a directed path originating from node~$u_1$.

Furthermore, after~$j$ steps each one of the nodes~$u_1,\dots,u_{k+1-(j+1)}$ has one child
with a height value of~$0$ and one child with a height value that is two less than its own. This implies that after the
$(j+1)$-st activation, the height value of each of the nodes will decrease by one. This establishes the part of the
claim that refers to the height values, and also the fact that after the $(j+1)$-st step, nodes
$u_1,\dots,u_{k+1-(j+2)}$ will be enabled for a height update.

It remains to show that node~$u_{k+1-(j+1)}$ will be enabled for a height update after the $(j+1)$-st step. Note that
node~$u_{k+1-j}$ is enabled for a height update after~$j$ steps, and therefore after the $(j+1)$-st step its height
value will have decreased by at least one. Also, as we just proved, after the $(j+1)$-st step the height value of its
father $u_{k+1-(j+1)}$ will have decreased by exactly one. Therefore, the latter will still be enabled for a height
update.
\end{proof}
\qed
\end{proof}



==> misc.tex <==

\section{Misc}

\begin{tabular}{lll}
\begin{minipage}{0.07\textwidth}
 (\textbackslash /)
\\( . .)'
\\(")(")
\end{minipage}
&
\begin{minipage}{0.63\textwidth}
\textbf{WARNING: Stuff in this subsection is unfinished, redundant, not completely correct, potentially useful, or any
combination thereof. Not to be considered as part of The Proof.}
\end{minipage}
&
\begin{minipage}{0.07\textwidth}
 (\textbackslash /)
\\( . .)'
\\(")(")
\end{minipage}
\end{tabular}

\begin{lemma}
 If heights are decreasing eventually the tree is balanced.

*** Redundant because of Lemma~\ref{lem:stablestate} *** Proof may be incorrect (assumes that when $m$ is swapped out of
the children set of $n$ it happens because $n$ is the target of a swap, but it could also be because $n$ is the source
of a swap) but may be fixable and possibly useful ***
\end{lemma}
\begin{proof}
A node cannot infinitely decrease its height.
The height of a leaf is eventually one (as soon as it executes $A1$).
A non leaf node $n$ is the root of a subtree containing leaves; eventually $h(n) \geq 2$.

Let's consider an execution where $A1$ is executed infinitely often.
As the number of nodes is finite, at least a node executes $A1$ infinitely often.
Let $n$ be a non leaf node that infinitely often execute $A1$.
As heights are decreasing $A1$ is executed only if $h(n)-h(max(n))>\alpha$.
Thus each time $n$ executes $A1$ its height decreases.
It follows that $n$ infinitely decreases its height.
This is a contradiction so no execution can execute $A1$ infinitely often.

Let's consider an execution where $A2$ is executed infinitely often.
Each time $A2$ is executed, a swap is performed.
Given that each swap has exactly one source and one target and that the number of nodes is finite, at least a node is
the target of an infinity of swaps.
Let $n$ be a node that is infinitely often the target of a swap.
As the number of nodes is finite, $n$ will eventually ``receive'' at least a node infinitely often.
Let $m$ be such a node.
Let $r$ be the first round where $n$ receives $m$ and $r''$ the next round where $n$ receives $m$.
During round $r$, $m$ is not the greatest children of $n$:
$$h(n)_r > h(m)_r + 1$$
Inbetween there is a round $r'$ ($r<r'<r''$) such that $m$ has been swapped out of $n$ subtree.
To have $m$ swapped out, it has to be the greatest child of $n$ during round $r'$:
$$h(n)_{r'} = h(m)_{r'} + 1$$
So between round $r$ and $r'$, $m$ became the greatest child of $n$.
As heights are decreasing $h(m)_r \geq h(m)_{r'}$.
We have $h(n)_r > h(m)_{r'} + 1$ and thus:
$$h(n)_r > h(n)_{r'}$$
If $n$ receives $m$ twice then the height of $n$ decreased inbetween.
If $n$ receives $m$ infinitely often, the height of $n$ infinitely decreases.
This is a contradiction so no execution can execute $A2$ infinitely often.

If heights are decreasing, for each execution there is a round such that no action will be executed anymore.
At this time both guards $G1$ and $G2$ are false for all nodes.
As a consequence all nodes are balanced.
Thus the tree is balanced.\cqfd
\end{proof}

\begin{definition}[Bad edges]
 In a given configuration $\conf{t}$, a directed edge $(u,v)$ is a \emph{bad edge} if $h_u(t)\leq h_v(t)$.
\end{definition}


We distinguish two phases in the execution of the algorithm. The end of the first phase is demarcated by the
extinction of bad edges in the system. In the second phase, nodes become balanced and their height variables attain the
correct values.

\begin{lemma}[Phase 1] \label{lem:ph1}
 Starting from an arbitrary configuration, the system no longer contains bad edges after at most $O(n)$ rounds.
\end{lemma}

\begin{lemma}[Phase 2] \label{lem:ph2}
 Starting from a configuration without bad edges, every node is balanced and contains correct height information after
at most $O(n)$ rounds.
\end{lemma}



\begin{subsubsection}{Proof of Lemma~\ref{lem:ph1}}

In any configuration $\conf{t}$, the bad edges partition the set of nodes into a number of subsets, which we call
\emph{subtrees}. Each subtree induces a maximal weakly connected directed subgraph of the original tree that contains no
bad edges.

\begin{claim}
 A swap operation cannot change the partition of nodes into subtrees.
\end{claim}
\begin{proof}
 Let $(u,v)$, $(w,x)$ be the two edges to be swapped, where $u$ is the father of~$w$. By definition of the swap guard,
the height variables of the four nodes must satisfy the following:
\begin{equation} \label{eq:swapheights}
h_v<h_x=h_w-1=h_u-2 \enspace.
\end{equation}
Therefore, $(u,v)$, $(w,x)$, and $(u,w)$ are not bad edges and all four nodes belong to the same subtree~$T$ before the
swap. 

Now, in view of (\ref{eq:swapheights}), the newly created edges $(u,x)$ and $(w,v)$ are not bad edges, and since a swap
does not affect the values of any height variables, the bad edges in the resulting configuration are exactly the same as
the bad edges in the original configuration.

Finally, the subtree~$T$ remains weakly connected, as any connecting path that was previously using edge $(w,x)$ can
replace it by the edges $(w,u)$ and $(u,x)$, and any connecting path that was previously using edge $(u,v)$ can replace
it by edges $(u,w)$ and $(w,v)$.
\end{proof}

\begin{claim}
 A height update operation on a node that is not the endpoint of a bad edge does not change the set of bad edges.
\end{claim}
\begin{proof}

\end{proof}
 
\end{subsubsection}



==> roundcompl.tex <==

\section{Round Complexity}

\begin{definition}[Leaf components]
 Let~$b$ be a bad node in~$\confext{t}$. $\mathcal{T}_b(t)$ is a \emph{leaf component} if for all
$u\in\mathcal{T}_b(t)$, $\children{u}(t)$ contains no bad nodes.
\end{definition}

\begin{lemma} \label{lem:leafcompstruct}
 Let~$\conf{t}\longrightarrow_A\conf{t'}$ be an execution step in Phase~1 (i.e., there is at least one bad
node in~$\conf{t}$), and let~$\mathcal{T}_b(t')$ be a leaf component in~$\conf{t'}$. Then, the following hold:
\begin{enumerate}
 \item If $b$ is bad in~$\conf{t}$ and the subtree of~$b$ in~$\conf{t}$ does not contain other bad nodes, then
$\mathcal{T}_b(t)$ is a leaf component in~$\conf{t}$, $b$ is not activated during
step~$\conf{t}\longrightarrow_A\conf{t'}$ and $\mathcal{T}_b(t)=\mathcal{T}_b(t')$.
 \item If $b$ is bad in~$\conf{t}$ and the subtree of~$b$ in~$\conf{t}$ contains at least one other bad node, or if $b$
is not bad in~$\conf{t}$, then there exists a leaf component~$L$ in~$\conf{t}$ such that $L\subset\mathcal{T}_b(t')$.
\end{enumerate}
\end{lemma}
\begin{proof}
 Coming. \qed
\end{proof}


\begin{lemma} \label{lem:leafcompincr}
 Let $\confext{t_1}$, $\confext{t_2}$ be the starting and final, respectively, extended configurations of one execution
round. Then the size of the smallest leaf component in~$\confext{t_2}$ is strictly larger than the size of the smallest
leaf component in~$\confext{t_1}$.
\end{lemma}
\begin{proof}
 Let $\tilde{\mathcal{C}}_0\equiv\confext{t_1},\tilde{\mathcal{C}}_1,\dots,\tilde{\mathcal{C}}_r\equiv\confext{t_2}$ be
the sequence of configurations in the round under consideration ($r\geq 1$). Let~$L_r$ be a smallest leaf component
in~$\tilde{\mathcal{C}}_r$.

Successive applications of Lemma~\ref{lem:leafcompstruct} for
steps~$\tilde{\mathcal{C}}_{r-1}\longrightarrow\tilde{\mathcal{C}}_r,
\tilde{\mathcal{C}}_{r-2}\longrightarrow\tilde{\mathcal{C}}_{r-1}, \dots,
\tilde{\mathcal{C}}_{0}\longrightarrow\tilde{\mathcal{C}}_1$ yield, for each extended
configuration~$\tilde{\mathcal{C}}_i$, a corresponding leaf component~$L_i$ such that $L_0\subseteq
L_1\subseteq\dots\subseteq L_r$. Moreover, at least one of these containments is strict: Otherwise,
Lemma~\ref{lem:leafcompstruct} would imply that the bad node which is the root of component~$L_0$
in~$\tilde{\mathcal{C}}_0$ is never activated or neutralized in the course of one round. We have then that
$|L_0|<|L_r|$ and the proof is complete. \qed
\end{proof}


\begin{corollary}
 Phase~1 is completed in at most~$n$ rounds.
\end{corollary}
\begin{proof}
 Immediate from Lemma~\ref{lem:leafcompincr} and the fact that in any extended configuration, the size of the smallest
leaf component is at least~$1$ and at most~$n+1$. \qed
\end{proof}

\begin{conjecture}
 Phase~2 is completed in~$\calO(n)$ rounds.
\end{conjecture}


